CuttleSys: Data-Driven Resource Management forInteractive Applications on Reconfigurable Multicores

Multi-tenancy for latency-critical applications leads to re-source interference and unpredictable performance. Core reconfiguration opens up more opportunities for colocation,as it allows the hardware to adjust to the dynamic performance and power needs of a specific mix of co-scheduled applications. However, reconfigurability also introduces challenges, as even for a small number of reconfigurable cores, exploring the design space becomes more time- and resource-demanding. We present CuttleSys, a runtime for reconfigurable multi-cores that leverages scalable and lightweight data mining to quickly identify suitable core and cache configurations for a set of co-scheduled applications. The runtime combines collaborative filtering to infer the behavior of each job on every core and cache configuration, with Dynamically Dimensioned Search to efficiently explore the configuration space. We evaluate CuttleSys on multicores with tens of reconfigurable cores and show up to 2.46x and 1.55x performance improvements compared to core-level gating and oracle-like asymmetric multicores respectively, under stringent power constraints.

==> algo_details.tex <==
\section{Combine with Algorithms}
For an N core system, small and big cores are considered equal in number i.e N/2 small cores and N/2 big cores. The runtime is divided into 100ms comprising of phases: sampling, surrogate fitting, thread mapping and steady state, the order of which depends on whether 2-step or 1-step algorithm is used to find the best configuration to be run in the final steady state. As the sampling interval is increased, the accuracy of the samples is improved but the system has to run in a sub-optimal configuration for a longer period of time. Thus, we choose to sample an application in a particular configuration for 1 ms.  
\subsection{Two-step Algorithms}
The 2-step algorithm first determines the mapping of threads onto the cores. The greedy algorithm described in section ?? requires sampled throughput and power values of all threads in a fully provisioned big core and small core i.e 4 lanes active and 2 lanes in all pipeline sections respectively. Since we have N/2 big cores and N/2 small cores, this sampling can be done in parallel. First half of the applications run on the big core for 1 ms while the other half is running on the big core and vice versa in the next 1 ms. By the end of 2ms, the required samples of all applications on the big core as well as the small are obtained. This phase of sampling involves migration of threads from big cores to small cores. In order to avoid considering the overhead of migration, we assume that no useful work is done in the 2 ms. In the next phase of thread mapping, based on the greedy heuristic, applications are mapped onto big/small cores. The runtime manager checks if for this mapping the power consumed by the applications in under the power constraint and if yes, the applications are run in this configuration for the remainder of 98 ms of the time slice. If the power constraint is violated, the cores need to be deconfigured to the best configuration which would be given by the optimization algorithm.



The optimization algorithm (GA/DDS) requires $B_{i,j} (P_{i,j}), j = 8, ..., 34$ for applications scheduled on big cores while $B_{i,j} (P_{i,j}), j = 0, ..., 7$ for applications scheduled on small cores. Reduced sampling technique, 3MM3, along with surrogate fitting is implemented to obtain all the 27 sampled values for the configurations 8, ..., 34 for applications scheduled on big cores. 3MM3 requires 9 specific configurations to be sampled which includes the (4,4,4) configuration, that is already sampled in the first phase. Replicated sampling (discussed in section ??) with eight replicates is applied to obtain the required 8 samples with each configuration being sampled for a total of 1 ms. Sampling of all the N/2 applications mapped on the big cores is done in parallel on the available N/2 big cores. For applications mapped on to the small core, only 8 samples are needed which is done in parallel on the N/2 small cores and simultaneously with the sampling on the big cores. The sampled points from the big core are used to generate a surrogate response for throughput and power for each application using the technique described in section ??. The applications do some useful work (execute instructions) in this stage though not in an optimal configuration which are accounted in the overall performance. ( how do we explain reconfiguring overhead). 
With all the $B_{i,j}$ and $P_{i,j}$ for all applications and needed configurations (applications on big cores only need the configurations on big cores and while those on the small cores only need the configurations on the small cores), parallel DDS/GA algorithm (Section ??) is run on all the N cores of the system. The number of iterations (or population \& generations) for which DDS (or GA) is run has a trade off with the quality of solution and the time utilized by the algorithm in which no work is done by the applications. 

Parallel DDS algorithm is chosen to run for 40 iterations with iteration step exploring ten points in the design space i.e setting $pointPerIteration = 10$ and $maxIter = 40$. Thus overall in an N-core system, $N * 400$ points are explored by the DDS algorithm. GA is run with a population of 20 for 25 generations on each core. The cores are deconfigured to the best solution obtained at the end the algorithm and are run in steady state for the remainder of 89 ms. Serial DDS and GA algorithm are run on real machine (describe machine) for 400 iterations and 25 generations with 20 population which takes about 0.9 ms. The load in the algorithm is pretty balanced fairly among the different threads. A synchronization overhead of 10\% is considered to account for the barriers used (need to synchronize for only $maxIter = 40$ times) in the parallel program (Figure ??).

\subsection{One-step Algorithm}
The one-step algorithm as discussed in section ??, requires the $B_{i,j}$ and $P_{i,j}$ values for all configurations of each application. 3MM3 sampling design is used to reduce the sampling required on the big core. A set of N/2 applications are sampled on the big cores for the first 9 ms and then the other applications are sampled on the big cores for another 9 ms. The sampling on the small cores is done in parallel with that on the big cores as it requires only 8 samples (i.e only 8 ms). Replicated sampling approach is applied for all this sampling with 8 replicates. As the one-step suffers from the disadvantage that only few points explored are valid (satisfy the core constraint), to obtain a good quality solution one-step algorithm is run for $maxIter = 80$ iterations with $pointPerIteration = 10$. Thus for an N-core system, $N*800$ points are explored in this algorithm. Thus, it is considered to take twice the amount of time taken by the parallel DDS in two-step algorithm (as seen in section ??). During this sampling phase, though the cores are not optimal configuration, some useful work is done which is accounted towards the final performance. (how to explain migration overhead ??) At the end of iterations, based on the best solution, threads are mapped to the corresponding cores and the each core is reconfigured concurrently to the configuration given by the best solution. The system runs in steady state for the remainder of the 80 ms. 




==> background-flicker.tex <==
\subsection{Background on Flicker}
%NOTE: This section is basically summing up section 3, 4.2 and 4.3 from Flicker. 
This section provides a brief overview of the Flicker microarchitecture and optimization approach.  Refer to~\cite{flicker} for full details.

The Flicker core 
%microarchitecture  bridges the gap between fine-grain microarchitecture adaptation and core-level gating. The 
pipeline is power-gated at the granularity of horizontal pipeline slices called lanes, which permits changing the superscalar width.
%and size of associated memory structures. 
%allowing the rapid adaptation of the width of different pipeline regions to meet the power budget of the system.
In Flicker, lanes are implemented within three independently controllable pipeline regions: Front End, Execute, and Memory.
%and each region can have different number of lanes turned on. 
When a lane is deconfigured, the associated queues are downsized proportionally.

The Flicker system is geared toward the \emph{dark silicon} problem~\cite{} in which not all chip transistors can be powered on at once.  In Flicker, the general-purpose cores are provided with a power cap, which specifies the fraction of full power that can be used by these cores, the value of which depends on the allocation of overall chip power to general-purpose cores and accelerators.

To determine the number of lanes within each of the cores to power on according to the power budget,  Flicker's runtime system first characterizes application behavior to obtain the throughput and power values for each application running in different possible configurations of the Flicker cores. This online characterization comprises two parts: (1) running applications for short sampling periods; and (2) using surrogate surface fitting techniques to determine the required throughput and power values. 

During sampling, an application is run for equal short periods each with a different configuration. 
Since the Flicker core has 27 possible configurations, and the sampling interval is 1ms, 
%while the little core has 8 configurations. S
full sampling consumes a large fraction of an operating system time slice,  during which the system runs in sub-optimal configurations. To reduce the sampling overhead, a Fractional Factorial design \cite{wu:3MM3} called 3MM3 ("3 Minus Modulus 3") 
%, $3^{k-1}$ design (where k is the number of factors and 3 represents the number of levels of each factor) 
%The factors for our design are the 3 different pipeline sections each of which can have 3 values (2, 3 or 4). Thus, the number of samples required for the big core is reduced to 9.
reduces the number of samples to nine.

%In online sampling, the measured responses are not only a function of the change in microarchitecture but also of the temporal fluctuations in the application behavior. In order to reduce the effect of the temporal fluctuations, replicated sampling is used. In this approach, multiple smaller samples of each configuration are obtained at different points and then averaged to get the final sample for each configuration. (Write in more detail ?? or reference flicker). As the number of replicates are increased, temporal fluctuations are reduced but at the same time sample size of each replicate decreases which are susceptible to noise due to microarchitectural events like cache mises, branch predictions etc. and reconfiguration overhead becomes more prominent. As shown in [ref Flicker], eight replicates improves the accuracy significantly and thus is used in this work.

Surrogate models 
%$T(x_1, x_2, x_3)$ and $P(x_1, x_2, x_3)$ 
are constructed to approximate the throughput and power responses for the remaining 18 configurations that are not sampled.
%by the 3MM3 approach. 
An interpolating Radial Basis Function (RBF) response surface \cite{guttmann, Mueller12, Regis12, Regis2007SRBF, Regis04IEEE} with a polynomial tail is applied to the sampled points to obtain the throughput and power response models. A genetic algorithm then searches for the best possible solution.
%(more details ??)
